Half-metallic zigzag carbon nanotube dots

A comprehensive first-principles theoretical study of the electronic properties and half-metallic nature of finite zigzag carbon nanotubes is presented. Unlike previous reports, we find that all nanotubes studied present a spin-polarized ground state, where opposite spins are localized at the two zigzag edges in a long-range antifferomagnetic configuration. Relative stability analysis of the different spin states indicate that, for the shorter segments, spin-ordering should be present even at room temperature. The energy gap between the highest occupied and the lowest unoccupied molecular orbitals of the finite systems is found to be inversely proportional to the nanotubes segments length, suggesting a route to control their electronic properties. Similar to the case of zigzag graphene nanoribbons, half-metallic behavior is obtained under the influence of an external axial electric field.

==> Makefile <==
.SUFFIXES: $(SUFFIXES) .dvi .ps .bib .tex .bbl .pdf

    PAPER_ROOT = Finite-CNT

  AIX_PSVIEWER = ghostview
Linux_PSVIEWER = ghostview
SunOS_PSVIEWER = ghostview

INFILES =  Finite-CNT.tex \
#	fkt.eps \
#	skw.eps


# PICTURES = 
#
# A very cool hack to "do the right thing":
       PSVIEWER = ${$(OS)_PSVIEWER}
#
#
# standard rules:
#
.dvi.ps:
	touch $*.ps
	/bin/rm $*.ps
	@echo "compiling $*"
	dvips -t a4 -o $*.ps $<

.ps.pdf:
	touch $*.pdf
	/bin/rm $*.pdf
	@echo "compiling $*"
	ps2pdf $< $*.pdf 

all:: ${PAPER_ROOT}.view

outline:: ${OUTLINE}.view

gs:: ${PAPER_ROOT}.psview

print: ${PAPER_ROOT}.ps  ${PAPER_ROOT}.pdf
print_outline: ${OUTLINE}.ps
	lpr ${OUTLINE}.ps

${PAPER_ROOT}.dvi: ${INFILES} ${PAPER_ROOT}.bib ${PICTURES}
	latex ${PAPER_ROOT}
	bibtex ${PAPER_ROOT}
	latex ${PAPER_ROOT}
	latex ${PAPER_ROOT}

${OUTLINE}.dvi: ${OUTLINE}.tex ${OUTLINE}.bib ${PICTURES}
	latex ${OUTLINE}
	bibtex ${OUTLINE}
	latex ${OUTLINE}
	latex ${OUTLINE}
	chmod 664 ${OUTLINE}.blg ${OUTLINE}.bbl ${OUTLINE}.aux ${OUTLINE}.dvi ${OUTLINE}.log

${PAPER_ROOT}.psview: ${PAPER_ROOT}.ps
	${PSVIEWER} ${PAPER_ROOT}.ps

${PAPER_ROOT}.view: ${PAPER_ROOT}.dvi
	xdvi ${PAPER_ROOT}

${OUTLINE}.view: ${OUTLINE}.dvi
	xdvi ${OUTLINE}

clean::
	/bin/rm -f *.aux *.log *.bbl *.blg *.dvi *~



